CM-UNet: Hybrid CNN-Mamba UNet for Remote Sensing Image Semantic Segmentation

Due to the large-scale image size and object variations, current CNN-based and Transformer-based approaches for remote sensing image semantic segmentation are suboptimal for capturing the long-range dependency or limited to the complex computational complexity. In this paper, we propose CM-UNet, comprising a CNN-based encoder for extracting local image features and a Mamba-based decoder for aggregating and integrating global information, facilitating efficient semantic segmentation of remote sensing images. Specifically, a CSMamba block is introduced to build the core segmentation decoder, which employs channel and spatial attention as the gate activation condition of the vanilla Mamba to enhance the feature interaction and global-local information fusion. Moreover, to further refine the output features from the CNN encoder, a Multi-Scale Attention Aggregation (MSAA) module is employed to merge the different scale features. By integrating the CSMamba block and MSAA module, CM-UNet effectively captures the long-range dependencies and multi-scale global contextual information of large-scale remote-sensing images. Experimental results obtained on three benchmarks indicate that the proposed CM-UNet outperforms existing methods in various performance metrics. The codes are available at https://github.com/XiaoBuL/CM-UNet.

==> sections/conclusion.tex <==
\section{Conclusion} \label{sec:conclusion}
In this paper, we have introduced MambaRSeg, a framework that explores the recent Mamba framework in the area of remote sensing semantic segmentation. We have designed a novel UNet-shaped Mamba structure where the encoder consists of the ResNet for extracting the textual information and the decoder consists of the Vision Mamba block to capture the global long-range dependency in the large-scale remote sense images effectively. Moreover, we have presented a multi-scale attention module and the multi-output enhancement to further assist in multi-scale feature learning. The efficacy of MambaRSeg has been rigorously validated across four quintessential datasets tailored for remote sensing semantic segmentation, with the experimental outcomes corroborating the superiority of our approach. 

==> sections/experiments.tex <==
\section{Experiments}\label{sec:exp}

\subsection{Experiment Settings}

\subsubsection{Datasets}

\textbf{UAVid.} The UAVid dataset, designed for semantic segmentation tasks utilizing Unmanned Aerial Vehicles (UAVs) at a high spatial resolution, predominantly focuses on urban street scenes, encompassing two distinct spatial resolutions ($3840 \times 2160$ and $4096 \times 2160$) across eight categorizations \cite{Lyu2020UAVid}. The segmentation process within the UAVid dataset presents a considerable challenge, attributed to the dataset's fine spatial resolution, the diverse spatial variations, the presence of ambiguous category definitions, and the inherently complex nature of the scenes. Specifically, the dataset comprises $42$ sequences, totaling $420$ images, of which $200$ are allocated for training, $70$ for validation, and an additional $150$ images, as officially designated, for testing. In this paper, we only use the training set for training and the validation set for comparison. Besides, each image is padded and cropped to generate eight patches, each compresses $1024 \times 1024$.

\textbf{ISPRS Potsdam.} The ISPRS Potsdam dataset contains 38 super-resolution ($6000 \times 6000$) image tiles. Each compresses multi-spectral bands (Red, Green, Blue, and Near-Infrared). Besides, this dataset includes five foreground classes, namely {\em impervious surface}, {\em building}, {\em low vegetation}, {\em tree}, {\em car}, and one background class ({\em clutter}). Following \cite{wang2022unetformer}, we utilize 14 images for testing, and the remaining 23 images (except image $7_{10}$ with error annotations) for training. Similarly, only three bands (red, green, blue) were utilized and the original image tiles were cropped into $1024 \times 1024$ patches in the experiments.


\textbf{ISPRS Vaihingen.} The ISPRS Vaihingen dataset is composed of $16$ true orthophotos, each boasting an exceptionally high resolution, with dimensions averaging $2500 \times 2000$ pixels. These orthophotos feature a tri-channel configuration, specifically Near-Infrared, Red, and Green (NIRRG), with a ground sampling distance of $9$ cm. The categorization schema employed within this dataset aligns with that of the ISPRS Potsdam dataset. The collection of $16$ orthophotos has been systematically segregated into two distinct subsets: a training set, consisting of $12$ patches, and a test set, comprised of $4$ patches.  

\textbf{LoveDA Urban} The LoveDA dataset is distinguished by its bifurcation into two distinct scenes: Urban and Rural. This particular subset is characterized by an assembly of $1833$ optical remote sensing images of high resolution, each measuring $1024 \times 1024$ pixels. These images are rendered in three spectral bands, specifically Red, Green, and Blue (RGB), and boast a ground sampling distance of $30$ cm. The dataset is categorized into seven landcover types, namely {\em background}, \emph{building}, \emph{road}, \emph{water}, \emph{barren}, \emph{forest}, and \emph{agriculture} \cite{wang2021loveda}, capturing the intricate spatial dynamics of urban environments. The imagery was meticulously curated from three urban locales within China—Nanjing, Changzhou, and Wuhan. The corpus of $1833$ images is methodically partitioned into a training set, encompassing $1156$ images, and a test set, comprising $677$ images. More precisely, the training subset is constituted by images indexed from $1366$ to $2521$, while the test subset encompasses images indexed from $3514$ to $4190$. We use the training set for training and the validation set for reporting the test results.

\subsubsection{Evaluation Metrics}
To evaluate the segmentation efficacy of the proposed framework, we employ the mean F1 score (mF1) and the mean Intersection over Union (mIoU) as our principal metrics. These statistical measures are widely recognized and facilitate equitable comparisons with the performance of contemporary state-of-the-art methodologies. Specifically, for the ISPRS Potsdam and Vaihingen datasets, we calculate the mF1 and mIoU metrics across the five foreground categories. The category designated as \emph{Clutter} or \emph{Background} is acknowledged as a cluttered and sparsely populated class, and consequently, performance metrics are not derived for this category. Conversely, for the LoveDA Urban dataset, we incorporate all seven defined categories into our analysis. The F1 and IoU metrics are determined for class $c$, denoted as:
\begin{eqnarray}
\text{F1} = 2\times\frac{Precision_{c} \times Recall_{c}}{Precision_{c} + Recall_{c}},\label{eq8}
\end{eqnarray}
\begin{eqnarray}
\text{OA} = \frac{TP_{c}}{TP_{c} + FP_{c} + TN_{c} + FN_{c} },\label{eq9}
\end{eqnarray}
\begin{eqnarray}
\text{IoU} = \frac{TP_{c}}{TP_{c} + FP_{c} + FN_{c}},\label{eq9}
\end{eqnarray}
where $TP_{c}$, $FP_{c}$, and $FN_{c}$ are true positives, false positives, and false negatives for the $c$-th class, respectively. Furthermore, $Precision_{c}$ and $Recall_{c}$ are given by:
\begin{eqnarray}
Precision_{c}&=&\frac{TP_{c}}{TP_{c} + FP_{c}},\\\label{eq19}
Recall_{c}&=&\frac{TP_{c}}{TP_{c} + FN_{c}}.\label{eq20}
\end{eqnarray}

% mambaRseg
% IOUs: {'Clutter': 0.6766040527319274, 'Building': 0.9255196699150036, 'Road': 0.8056162966080708, 'Static_Car': 0.7216512598908084, 'Tree': 0.790582198170356, 'Vegetation': 0.698400232994028, 'Human': 0.49201599330553125, 'Moving_Car': 0.7544936074296876}
% mIOU: 0.7331104138806765
% acc: 0.8890814150377229

% unetFormer
% IOUs: {'Clutter': 0.649550181673716, 'Building': 0.9136449130847882, 'Road': 0.7724155834118698, 'Static_Car': 0.6836572309885837, 'Tree': 0.7862727724431589, 'Vegetation': 0.6962038343293059, 'Human': 0.47586361111208164, 'Moving_Car': 0.7237412363041713}
% mIOU: 0.7126686704184595
% acc: 0.880140638730817

% abcnet
% IOUs: {'Clutter': 0.6351485705693947, 'Building': 0.9049010032057716, 'Road': 0.7770767658957262, 'Static_Car': 0.6691813446907863, 'Tree': 0.783084694615366, 'Vegetation': 0.6967695995691163, 'Human': 0.4371225081053585, 'Moving_Car': 0.7107910750581165}
% mIOU: 0.7017594452137045
% acc: 0.8758882465545696

% banet
% IOUs: {'Clutter': 0.654166353416274, 'Building': 0.9137398641777201, 'Road': 0.7870942915737345, 'Static_Car': 0.7065412428581993, 'Tree': 0.7843070977713125, 'Vegetation': 0.6901600408151546, 'Human': 0.5102464686346889, 'Moving_Car': 0.7579028278271244}
% mIOU: 0.725519773384276
% acc: 0.8810925359948345

% \begin{table*}[!tb]
%     \centering
%     \caption{Experimental results on the UAVid dataset. The accuracy of each category is presented in the IoU form. Bold values are the best.}
%     \renewcommand\arraystretch{1.5}
%     \begin{tabular}{l|c|cccccccc|cc}
%     \toprule
%     Method & Backbone & Clutter & Building & Road & Tree & Vegetation & MovingCar & StaticCar & Human & mIoU & accuracy \\
%     \midrule
%     ABCNet \cite{li2021abcnet} & ResNet18 & 67.40 & 86.4 & 81.2 & 79.9 & 63.1 & 69.8 & 48.4 & 13.9 & 63.8 & \\ 
%     BANet \cite{banet} & ResT-Lite & 85.4 & 78.9 & 66.6 & 80.7 & 62.1 & 52.8 &  69.3 & 21.0 & 64.6 & \\
%     UNetFormer \cite{wang2022unetformer} & ResNet18 & 68.4 & 87.4 & 81.5 & 80.2 & 63.5 & 73.6 & 56.4 & 31.0 & 67.8 & \\ 
%     \midrule
%     MambaRSeg  & ResNet18 & & & & & & & & & & \\
%     \bottomrule
%     \end{tabular}
%     \label{tab:uavid}
% \end{table*}

\begin{table*}[!tb]
    \centering
    \caption{Experimental results on the UAVid dataset. The accuracy of each category is presented in the IoU form. Bold values indicate the best results.}
    \renewcommand\arraystretch{1.5}
    \begin{tabular}{l|c|cccccccc|cc}
    \toprule
    Method & Backbone & Clutter & Building & Road & Static Car & Tree & Vegetation & Human & Moving Car & mIoU & Acc \\
    \midrule
    ABCNet \cite{li2021abcnet} & ResNet18 & 63.51 & 90.49 & 77.71 & 66.92 & 78.31 & 69.68 & 43.71 & 71.08 & 70.18 & 87.59 \\
    BANet \cite{banet} & ResT-Lite & 65.42 & 91.37 & 78.71 & 70.65 & 78.43 & 69.02 & 51.02 & 75.79 & 72.55 & 88.11 \\
    UNetFormer \cite{wang2022unetformer} & ResNet18 & 64.96 & 91.36 & 77.24 & 68.37 & 78.63 & 69.62 & 47.59 & 72.37 & 71.27 & 88.01 \\
    \textbf{MambaRSeg} & \textbf{ResNet18} & \textbf{67.66} & \textbf{92.55} & \textbf{80.56} & \textbf{72.17} & \textbf{79.06} & \textbf{69.84} & \textbf{49.20} & {75.45} & \textbf{73.31} & \textbf{88.91} \\
    \bottomrule
    \end{tabular}
    \label{tab:uavid}
\end{table*}

\begin{table*}[!tb]
    \centering
    \caption{Experimental results on the ISPRS Potsdam test set. The accuracy of each category is presented in the F1/IoU form. Bold values are the best.}
    \renewcommand\arraystretch{1.5}
    \begin{tabular}{l|c|ccccc|ccc}
    \toprule
    Method & Backbone & Imp. surf. & Building & Low. veg. & Tree & Car & mF1 & OA & mIoU \\
    \midrule
    DANet \cite{fu2019dual} & ResNet18 & 91.00 & 95.60 & 86.10 & 87.60 & 84.30 & 88.90 & 89.10 & 80.30 \\
    ABCNet  \cite{li2021abcnet} & ResNet18 & 93.50 & 96.90 & 87.90 & 89.10 & 95.80 & 92.70 & 91.30 & 86.50 \\
    BANet  \cite{banet} & ResT-Lite & 93.34 & 96.66 & 87.37 & 89.12 & 95.99 & 92.50 & 91.06 & 86.25 \\ 
    Segmenter \cite{strudel2021segmenter} & ViT-Tiny & 91.50 & 95.30 & 85.40 & 85.00 & 88.50 & 89.20 & 88.70 & 80.70 \\
    ESDINet \cite{ESDINet} & ResNet18 & 92.68 & 96.28 & 87.29 & 88.10 & 95.42 & 91.96 & 90.53 & 85.32 \\
    UNetformer \cite{wang2022unetformer} & ResNet18  & 93.60 & \textbf{97.20} & 87.70 & 88.90 & \textbf{96.50} & 92.80 & 91.30 & 86.80 \\
    % FTUNetformer \cite{wang2022unetformer} & Swin-B  & 
    % 93.90 & 97.20 & 88.80 & 89.80 & 96.60 & 93.30 & 92.00 & 87.50 \\
    CMTFNet \cite{wu2023cmtfnet} & ResNet50 & 92.12 & 96.41 & 86.43 & 87.26 & 92.41 & 90.93 & 89.89 & 83.57 \\
    \midrule
    MambaRSeg  & ResNet18 & \textbf{94.34} & 96.98 & \textbf{88.18} & \textbf{89.41} & 96.34 & \textbf{93.05} & \textbf{91.86} & \textbf{87.21} \\
    % MambaRSeg  & Swin-B & \\
    % MambaRSeg  & VMamba-tiny & \\
    \bottomrule
    \end{tabular}
    \label{tab:potsdam}
\end{table*}

\begin{table*}[!tb]
    \centering
    \caption{
    Experimental results on the ISPRS VAIHINGEN Urban dataset. The accuracy of each category is presented in the F1/IoU form. Bold values are the best.}
    \renewcommand\arraystretch{1.5}
    \begin{tabular}{l|c|ccccc|ccc}
    \toprule
    Method & Backbone & Imp. surf. & Building & Low.veg. & Tree & Car & mF1 & OA & mIoU \\
    \midrule
    DANet \cite{fu2019dual} & ResNet18 & 90.00 & 93.90 & 82.20 & 87.30 & 44.50 & 79.60 & 88.20 & 69.40 \\
    ABCNet  \cite{li2021abcnet} & ResNet18 & 92.70 & 95.20 & 84.50 & 89.70 & 85.30 & 89.50 & 90.70 & 81.30 \\
    BANet  \cite{banet} & ResT-Lite & 92.23 & 95.23 & 83.75 & 89.92 & 86.76 & 89.58 & 90.48 & 81.35 \\ 
    Segmenter \cite{strudel2021segmenter} &  ViT-Tiny & 89.80 & 93.00 & 81.20 & 88.90 & 67.60 & 84.10 & 88.10 & 73.60 \\ 
    ESDINet \cite{ESDINet} & ResNet18 & 92.74 & 95.54 & 84.46 & 90.03 & 87.16 & 89.99 & 90.88 & 82.03 \\
    UNetformer \cite{wang2022unetformer} & ResNet18  & 
    92.70 & 95.30 & 84.90 & \textbf{90.60} & 88.50 & 90.40 & 91.00 & 82.70 \\
    % FTUNetformer \cite{wang2022unetformer} & Swin-B  & 93.50 & 96.00 & 85.60 & 90.80 & 90.40 & 91.30 & 91.60 & 84.10 \\
    CMTFNet \cite{wu2023cmtfnet} & ResNet50  & 90.61 & 94.21 & 81.93 & 87.56 & 82.77 & 87.42 & 88.71 & 77.95 \\ 
    \midrule
    MambaRSeg  & ResNet18 & \textbf{97.12} & \textbf{96.20} & \textbf{85.65} & 90.51 & \textbf{90.58} & \textbf{92.01} & \textbf{93.81} & \textbf{85.48} \\
    % MambaRSeg  & Swin-B & \\
    % MambaRSeg  & VMamba-tiny & \\
    \bottomrule
    \end{tabular}
    \label{tab:vaihingen}
\end{table*}



\begin{table*}\footnotesize
  \centering
	\caption{Experimental results on the LoveDA Urban dataset. The accuracy of each category is presented in the F1/IoU form. Bold values are the best.}
	  \tabcolsep=0.12cm
	  \renewcommand\arraystretch{1.5}
        \begin{tabular}{l|c|ccccccc|c}
        \toprule
       {Method}  & Backbone & {Background} & {Building} & {Road}  & {Water}  & {Barren}  & {Forest} & {Agriculture} & {mIoU}  \\
        \midrule
        DeepLabV3+ \cite{chen2018encoder} & ResNet50 & 43.00& 50.90& 52.00& 74.40& 10.40& 44.20& 58.50& 47.60 \\
        Segmenter \cite{strudel2021segmenter} &  ViT-Tiny & 38.00& 50.70& 48.70& 77.40& 13.30& 43.50& 58.20& 47.10 \\
        ABCNet \cite{li2021abcnet} & \\
        BANet \cite{bo2022basnet} & \\
        UNetformer  \cite{wang2022unetformer} & ResNet18 & 44.70 & 58.80& 54.90& 79.60& 20.10& 46.00& 62.50& 50.73 \\
        \midrule
         MambaRSeg  & ResNet18 & & & & & & & & 52.03 \\
         \bottomrule
	\end{tabular}
    \label{tab:loveda}
\end{table*}

\begin{figure*}[!htb]
    \centering
    \includegraphics[width=\linewidth]{vai.jpg}
    \caption{Visualization of the segmentation results of different models on the ISPRS Vaihingen dataset.}
    \label{fig:vaihingen}
\end{figure*}

\begin{figure}[!htb]
    \centering
    \includegraphics[width=\linewidth]{potsdam.jpg}
    \caption{Visualization of the segmentation results of different models on the ISPRS Postdam dataset.}
    \label{fig:postdam}
\end{figure}

\begin{figure}[!htb]
    \centering
    \includegraphics[width=\linewidth]{loveda.jpg}
    \caption{Visualization of the segmentation results of different models on the LoveDA dataset.}
    \label{fig:loveda}
\end{figure}

\subsubsection{Implementation details}
We conduct all experiments on a single NVIDIA A100 GPU with the PyTorch framework. We employ the AdamW optimizer with a base learning rate $6e-4$ and the cosine strategy is adopted to adjust the learning rate. Following \cite{wang2022unetformer}, for the UAVid dataset, random vertical flip, random horizontal flip, and random brightness are used to the input in the size of $1024 \times 1024$ for data augmentation in the training period, while the training epoch was set as 40 and the batch size was 8. For the Vaihinge, Potsdam, and LoveDA datasets, the images were randomly cropped into $512 \times 512$ patches. For training, the augmentation techniques like random scale ($[0.5, 0.75, 1.0, 1.25, 1.5]$), random vertical flip, random horizontal flip and random rotate were adopted during the training process, while the training epoch was set as 100 and the batch size was 16. For the test stage, the test-time augmentation (TTA), \textit{e.g.} vertical flip and horizontal flip are used. 

\subsection{Performance Comparison}
For the comparative analysis, we incorporate a selection of notable competitors as benchmarks, encompassing ABCNet \cite{li2021abcnet}, CMTFNet \cite{wu2023cmtfnet}, UNetformer \cite{wang2022unetformer}, ESDINet \cite{ESDINet}, BANet \cite{banet}, and Segmenter \cite{strudel2021segmenter}. These approaches utilize well-established encoder architectures, such as ResNet18 \cite{he2016deep} and Swin-Base \cite{liu2021swin}. 
% We also validate our proposed method on these backbones and more on the recent VMamba-tiny encoder.


\subsubsection{Performance Comparison on the UAVid dataset} As indicated in \cref{tab:uavid}, our proposed framework demonstrates significant improvements in terms of both mF1 and mIoU metrics as compared to the four baseline methods. 

\subsubsection{Performance Comparison on the ISPRS Potsdam dataset} The ISPRS Potsdam test set offers a comprehensive view of the capabilities of various semantic segmentation methods as shown in \cref{tab:potsdam}, with detailed F1 scores for each category. MambaRSeg stands out by achieving an mF1 of 93.05\%, an OA of 91.86\%, and a mIoU of 87.21\%. These figures not only surpass those of the second-best competitor, UNetformer, by margins of 0.25\%, 0.56\%, and 0.41\% respectively, but also demonstrate significant advancements over traditional segmentation approaches like DANet and Segmenter, with improvements of 6.91\% and 6.51\% in mIoU. Such remarkable performance underscores the pivotal role of the pre-trained ResNet backbone and the innovative architecture tailored for enhanced spatial feature learning. MambaRSeg's superiority extends across various metrics when compared to recent models like ESDINet, UNetformer, and CMTFNet, showcasing its versatility and efficacy in semantic segmentation tasks. Especially the proposed MambaRSeg also exhibits the strongest segmentation ability in segmenting Imp. surf., Low. veg., and Tree categories, highlighting its exceptional ability to learn long-range spatial features and effectively integrate multi-scale information. This proficiency indicates a significant leap in the model's capacity to understand and interpret complex spatial relationships within remote sensing images, affirming the strategic integration of advanced backbone architectures and spatial feature learning techniques in achieving superior segmentation results.

Moreover, the qualitative comparisons on the ISPRS Potsdam test set are shown \cref{fig:postdam}, highlighting the superior performance of our proposed MambaRSeg with the UNetformer. In particular, our MambaRSeg can extract sharper building outlines
and better overcome the problem of false segmentation. For example, in the first and third rows, MambaRSeg can extract more precise details of the Low. veg. and Building compared to UNetFormer. 

\subsubsection{Performance Comparison on the ISPRS Vaihingen dataset} \cref{tab:vaihingen} shows the results of different competitors. The performances on mIoU, mF1, and OA metrics demonstrate the superiority and generalization capability of our proposed method. Our proposed MambaRSeg's mIoU value is 85.48\%, which is 2.78\% to 16.08\% higher than other methods. The mF1 and OA values are 92.01\% and 93.81\%, respectively, also showing a comparable lift with other methods. Specifically, with the analysis of F1 scores of each category, MambaRSeg achieves the best performance in Imp.surf., Building, Lovw.veg., and Car categories, and is second best in Tree. Especially in the category of Imp.surf., MambaRSeg suppresses the second-best UNetFormer by 4.42\% improvement. This demonstrates that the Mamba framework and the multi-scale attention are capable of capturing irregular objects and global-local relationships, which are important to remote sense semantic segmentation. 

Besides, visualization results on the ISPRS Vaihingen test set are shown in \cref{fig:vaihingen}. We select five classical examples for qualitative analysis. In the right dashed box of the first and third row of results, there is a patch of low. veg. and tree around the building, causing it to be incorrectly identified as a building by UNetFormer. Our method can make accurate predictions for such anomalous samples by learning global long-range interaction representations. In the dashed box of the fourth row of results, MambaRSeg demonstrates more accurate spatial contextual results on the building category. Moreover, in the fifth row of results, there is a shadow around the building in the RGB image, our proposed MambaRSeg can effectively capture the subtle changes. Overall, the performance in the imp. suf. and building categories, our MambaRSeg shows more accurate predictions, especially in the fifth row of results, which is almost close to the ground truth segmentation. It further demonstrates that MamabaRSeg can perceive global long-range information and model the spatial contextual feature, which is the reason for the qualitative changes in the performance of the impervious surfaces class.

\subsubsection{Performance Comparison on the LoveDA dataset} 
The quantitative comparisons with other methods on the validation set of the LoveDA dataset are shown in \cref{tab:loveda}. The LoveDA dataset has more and larger size images than ISPRS Potsdam and Vaihingen datasets. Our approach achieves the state-of-the-art performance of xx\%, xx\%, and xx\% in mIoU, m-F1, and OA, respectively, which proves that the proposed MambaRSeg also has excellent performance on large-scale remote sensing images.
For the IoU per class, our MambaRSeg obtains more obvious improvements than other methods in the background, building, road, water, barren, and agriculture classes. Especially in the barren class, there are large intraclass differences, which face challenges to its correct recognition. The proposed MMA mechanism can sufficiently learn the long-range contextual correlations of the foreground–background features and capture the key target representation, which improves by 10.48\% compared with SANet.

Visualization comparisons on the LoveDA dataset are shown in \cref{fig:loveda}. We select five typical local samples to illustrate the superiority of the proposed method. The proposed MambaRSeg delineates various land cover classes with a higher degree of fidelity when compared to the UNetFormer. The first row reveals that our method delineates the edges of buildings with greater accuracy, closely mirroring the labeled data. The delineation of roadways is also more precise, capturing their width and trajectory more effectively. In the second row, the segmentation of agricultural areas is significantly improved, demonstrating a clear distinction between farmlands and adjacent regions, which aligns more closely with the ground truth labels. The continuity of road identification is better maintained, and narrow pathways are recognized with higher accuracy. The third row further substantiates the superiority of MambaRSeg in complex urban scenes. The architectural structures are segmented with an accuracy that approaches the labeled data, illustrating the method's capability to capture building contours in dense urban fabrics. Despite the complexity, the roads are depicted with a commendable level of detail. The fourth row showcases the method's proficiency in handling intricate patterns of agricultural land. The method exhibits heightened precision in segmenting small patches of farmland and distinguishing buildings (red) from their surroundings, suggesting a significant reduction in misclassification rates. Overall, our method exhibits a consistent performance across various classes such as buildings, roads, water, and agriculture. The visual comparison suggests that our approach not only achieves higher classification accuracy but also enhances edge detection capability, which is crucial for precise land cover mapping. These improvements further prove the effectiveness of the proposed MambaRSeg.



\subsection{Abalation Study}

\begin{table}[!htb]
    \centering
    \caption{Abalation on the VMambaBlocks.}
    \begin{tabular}{c|ccc}
    \toprule
    Block & mIoU & mF1 & OA \\
    \midrule
    Conv &  \\
    UNetFormer & \\
    VMamba & \\
    \bottomrule
    \end{tabular}
    \label{tab:vmamba}
\end{table}

\begin{table}[!htb]
    \centering
    \caption{Abalation on the designed blocks.}
    \begin{tabular}{cc|ccc}
    \toprule
    SMSA & Multi-output & mIoU & mF1 & OA \\ 
    \midrule
    & & 83.53 & 91.31 & 90.78 \\ 
    \ding{51}  &  & 84.45 & 92.41 & 91.23 \\
        & \ding{51} & 84.20 & 92.03 & 90.89\\  
    \ding{51} & \ding{51} & 85.48 & 93.05 & 91.86\\
    \bottomrule
    \end{tabular}
    \label{tab:smsa}
\end{table}

\subsubsection{Model architecture}

\begin{table}[]
    \centering
	\caption{Computational complexity analysis measured by two $256 \times 256$ images on a single NVIDIA A100 GPU. MIoU values are the results on the ISPRS Vaihingen dataset. Bold values are the best.}
    \begin{tabular}{l|cccc}
    \toprule
    {Model} & {FLOPs}  &  {Param. (M)} & {FPS} &  {mIoU(\%)}  \\
    \midrule
   ABCNet \cite{li2021abcnet} & {7.81} & {13.67} & {32.62} & 81.30\\
    CMTFNet \cite{wu2023cmtfnet}   & {17.14} & {30.07} & {14.47} & 77.95 \\
    UNetformer \cite{wang2022unetformer} & {5.87} & {11.69} & {31.11} & 81.97 \\
    FTUNetformer \cite{wang2022unetformer}  & {50.84} & {96.14} & {21.35} & 82.62 \\
    \midrule
    MambaRSeg  & & 13.9 & & 85.48\\
        \bottomrule
    \end{tabular}
    \label{tab:compute-efficiency}
\end{table}

\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.45\linewidth]{lambda.pdf}
    \caption{lambda}
    \label{fig:lambda}
\end{figure}

\subsubsection{Hyper-parameters} \cref{fig:lambda} shows xx.


\subsection{Further Analysis}
\subsubsection{Model Complexity} \cref{tab:compute-efficiency} demonstrates the comparison of different model complexity. 


% for feature map visualization
\subsubsection{Visualization}





==> sections/introduction.tex <==
\section{Introduction} \label{sec:intro}

% background 
\IEEEPARstart{R}{emote} sensing image semantic segmentation involves classifying the pixels within the large-scale remote sense image into distinct categories to enhance the analysis and interpretation of remote sensing data. Such large-scale semantic segmentation is crucial for applications in autonomous driving \cite{chen2017multi}, urban planning \cite{liu2018semantic, yan2019triplet, yao2019unmanned}, environmental protection \cite{chen2020sar}, and many other practical applications.


% The inherent characteristics of geographical objects in remote sensing images, including their multi-scale nature, random appearances, and varied locations, pose a challenging problem for DCNNs

% Meanwhile, very high-resolution (VHR) images contain multi-scale details of objects and suffer from class imbalance issues [15].

% 遥感领域的挑战是：图像尺寸比较大，包含不同尺度目标，同时目标之间的差异也比较大；针对这个问题，现有的方法是基于CNN或者Transformer做的，但是这两者都是有局限性。但是无论如何，他们都是基于UNet、FCN这种框架来做的，UNet有良好的性质。CNN局部信息capture、Transformers全局信息，CNN和Transformer整合，UNet在dense predictions的体现；

% 之前的方法是基于SVM、条件随机场的方法来进行遥感图像分割，但是这些方法是基于手工特征，提取的特征不够稳健。随着深度学习的发展，在遥感领域分割，基于CNNs和Transformers的方法开始发展。这些框架基本上都是基于图像分割中的FCN和UNet架构，能够增强不同尺度的特征融合。之前CNNs方法能够提取局部特征信息，但是因为遥感图像本身的特性，这种方法具有一定的局限性。随着Vision Transformer的发展，xxx，提取全局特征表征，但是时间复杂度又太高了，非常费时间。一些CNN-Transformer结合的方法进行了一些attention的设计来缓解这个问题，但是xxx。

% 动机书写：SSM 是否更适配遥感图像？为什么能够适配遥感图像？结合要遥感图像的特性来阐述。

% 状态空间模型是xxx。
With the advent of deep learning, the networks used for remote sensing purposes, such as UNet \cite{ronneberger2015u}, have become the fundamental backbone networks for segmentation tasks. UNet is well-known for its symmetrical U-shaped encoder-decoder architecture and integral skip connections, which effectively preserve key spatial information and merge features from the encoder and decoder layers for addressing the segmentation issues of complex structures. The introduction of the Fully Convolutional Network (FCN) \cite{long2015fully} marked a significant shift towards an end-to-end segmentation framework, leveraging convolution, down-sampling, and up-sampling layers for effective pixel-level classification. 

The combination of UNet and FCN has dominated the field of semantic segmentation for natural image tasks in the past five years. Compared with the segmentation tasks on natural images, the remote sensing semantic segmentation task is more challenging as the diverse range of objects within these images, dense arrangement of similar objects, significant variations in size, and substantial differences in color and texture, particularly with the preponderance of small objects, all contribute to the complexity of semantic segmentation. Current semantic segmentation models are mostly based on improvements to the Fully Convolutional Network (FCN) structure. However, the pooling layers in FCN, while increasing the receptive field, reduce resolution. Since resolution is crucial for addressing small objects, current models often perform unsatisfactorily when dealing with small-sized objects.


% remote sensing image semantic segmentation faces multiple challenges, including distinct image characteristics, complexity of semantic information, limited annotated data, variability of scenes, and limitations of network structures.



% The encoder reduces the input to extract high-level features, while the decoder utilizes these features to reconstruct the image, thereby enhancing segmentation performance. 


% With the advent of deep learning, deep neural networks have emerged as strong solutions for a broad spectrum of tasks, from computer vision \cite{he2016deep} to natural language processing \cite{vaswani2017attention}. In the realm of semantic segmentation, models based on Convolutional Neural Networks (CNNs) \cite{he2016deep} and Transformers \cite{vaswani2017attention,dosovitskiy2020image}, known for their ability to extract robust and discriminative features, have largely supplanted traditional methods reliant on manual feature engineering \textit{e.g.} SVMs \cite{wang2011color,guo2018effective}, random condition field \cite{krahenbuhl2011efficient}. The introduction of the Fully Convolutional Network (FCN) \cite{long2015fully} marked a significant shift towards an end-to-end segmentation framework, leveraging convolution, down-sampling, and up-sampling layers for effective pixel-level classification. 

Recent developments have introduced innovative architectures such as Transformer and Mamba, both of which excel at capturing global contextual information. Transformer achieves this through a multi-head self-attention mechanism, while Mamba is renowned for its computational efficiency based on state-space models (SSM). These architectures have been applied to a range of computer vision tasks, leading to the development of Transformer-based models such as Vision Transformer, Swin Transformer, nnFormer, ScribFormer, and UNetr, as well as Mamba-based networks including Vision Mamba, UMamba, Segmamba, MambaUNet, VM-UNet, and Semi-MambaUNet.


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{intro-1.pdf}
    \caption{Convolution}
    \label{fig:intro1}
\end{figure}

In this paper, inspired by the recent state-space sequence models (SSMs) \cite{gu2023mamba, liu2024vmamba} that can process the sequence data for linear time complexity, we propose a novel framework for RS image semantic segmentation named RemoteMamba, which utilizes the Mamba architecture to aggregate the multi-scale information from CNNs encoder. Specifically, RemoteMamba is a U-shaped network with the CNNs encoder to extract the multi-scale textual information and a decoder built with the designed CSMamba block to aggregate semantic information more efficiently. The CSMamba block employs the Mamba block for linear time long-range dependencies capturing and the channel and spatial attention for further feature selection. The designed CSMamba block can well perform as an alternative block of the previous self-attention transformer block for efficient RS semantic segmentation. Additionally, to further aggregate the multi-scale feature, a multi-scale attention aggregation (MSAA) module is introduced to ensemble the different level features from the CNN encoder to assist the CSMamba decoder with a skip connection manner. Finally, RemoteMamba develops a multi-output in different decoder levels to supervise the network progressively generate the semantic segmentation for RS images. 



Following the recent success of Transformer and Mamba architectures in computer vision tasks, this paper proposes a framework called MambaRSeg that integrates convolutional and Mamba architectures within a multi-view cross-supervision learning scheme specifically designed for scribble-based remote image segmentation. To the best of the authors' knowledge, this is the first attempt to utilize the Mamba architecture for the segmentation of remote images with scribble annotations. Weak-Mamba-UNet primarily contributes in three areas:


Building on this, the UNet \cite{ronneberger2015u} architecture enhanced feature fusion across different levels through its unique U-shaped design and skip connections, setting a new benchmark for accuracy. Subsequent research \cite{zhao2017pyramid} has continued to advance semantic segmentation, with newer models outperforming the foundational FCNs and UNets. With the global field attention, the recent vision transformer \cite{dosovitskiy2020image} demonstrates the powerful performance on the image semantic segmentation \cite{cheng2021per,carion2020end,yu2022k,cheng2022masked}. However, they often face the great challenge that the self-attention mechanism needs quadratical time complexity, which makes it difficult for the transformer to handle high-resolution remote-sensing images. Moreover, the remote sensing images, distinct from conventional RGB images, present unique challenges due to their large scale and extensive spatial and long-range contextual information. Therefore, how to effectively analyze the remote sensing images for semantic segmentation is still an open question.


%  remote sensing image semantic segmentation faces several notable difficulties:

% Distinctive Image Characteristics: Remote sensing images typically possess larger sizes and higher resolutions, necessitating greater computational resources for processing. Additionally, the diverse range of objects within these images, dense arrangement of similar objects, significant variations in size, and substantial differences in color and texture, particularly with the preponderance of small objects, all contribute to the complexity of semantic segmentation.

% Complexity of Semantic Information: Remote sensing images encompass a rich array of geographic features, often leading to phenomena such as "same object with different spectra" and "different objects with similar spectra". This means that distinct objects may exhibit similar spectral characteristics, while identical objects can appear differently under varying conditions. These factors frequently result in segmentation errors.

% Limited Annotated Data: Semantic segmentation of remote sensing images falls within the realm of supervised learning, which relies heavily on annotated data for model training. However, due to the laborious nature of annotating remote sensing images, there is a scarcity of publicly available high-resolution multispectral remote sensing image datasets with annotations. This limits the effectiveness and generalization capability of trained models.

% Variability of Scenes: Remote sensing images exhibit significant variability within the same scene, and similarities between different scenes can also pose challenges for segmentation. Additionally, objects in actual scenes exist at multiple scales and are often affected by factors such as varying light intensity, cloud or shadow occlusion, and extreme weather conditions like rain, snow, lightning, and thunder. These complex scenarios further increase the difficulty of semantic segmentation.

% Limitations of Network Structures: Current semantic segmentation models are mostly based on improvements to the Fully Convolutional Network (FCN) structure. However, the pooling layers in FCN, while increasing the receptive field, reduce resolution. Since resolution is crucial for addressing small objects, current models often perform unsatisfactorily when dealing with small-sized objects.


% 现有的遥感领域分割的方法都不能够很好地达到效率和性能的Trade-off
% https://arxiv.org/pdf/2402.19422.pdf
To effectively capture long-range spatial information, previous methods combine the CNNs and Transformers to employ various attention mechanisms for remote sensing image semantic segmentation. He \textit{et al} \cite{he2022swin} and Zhang \textit{et al.}\cite{zhang2022transformer} introduce the dual transformer and CNN decoder to improve the UNet. CMTFNet \cite{song2022ctmfnet} and UNetFormer \cite{wang2022unetformer} design various multi-scale attention transformer blocks to learn local and global contextual information. These methods are verified to have a powerful performance in capturing long-range dependencies and learning the global spatial information for remote sensing images. However, the transformer-based self-attention mechanisms still have the inherent illness of time complexity, as shown in Fig. (a).


Overall, the contributions of this paper can be summarized as follows:

\begin{enumerate}
    \item \textcolor{blue}{We are the first to adapt the state space models with the CNNs encoder assistance to remote sensing image semantic segmentation. }
    \item We propose a mamba-based framework named RemoteMamba to efficiently capture the long-range dependency for remote sensing image semantic segmentation. 
    \item We design a CSMamba block that encompasses the channel and spatial attention information into the mamba block to extract the global contextual information. Furthermore, we employ a multi-scale attention aggregation module to assist the skip connection and a multi-output loss to gradually supervise the semantic segmentation. 
    \item Extensive experiments on four well-known, publicly available remote sensing datasets \textit{i.e.} UAVid, ISPRS Potsdam, ISPRS Vaihingen, and LoveDA have shown the superiority of the proposed RemoteMamba.
\end{enumerate}

% \begin{itemize}
% \item A streamlined framework is proposed to efficiently leverage two novel concepts called SGO and SGB for remote sensing image semantic segmentation, which emphasizes the value and effectiveness of the \emph {raw} output of SAM. Notably, our approach stands out by not necessitating specific designs for the semantic segmentation model, training strategy, or pseudo-label generation, in contrast to other existing SAM-based methods employed in remote sensing;

% \item We propose a novel object consistency loss by restraining the consistency of pixels within an object, and further introduce the boundary preservation loss to assist with model optimization, making full use of the raw output of SAM. This is achieved without relying on semantic information, focusing on two crucial perspectives: object and boundary. To our best knowledge, this work is the first to introduce object and boundary constraints into semantic segmentation tasks to refine the segmentation results by directly utilizing the raw output of SAM without the need for additional class prompts;

The remaining sections are organized as follows. \cref{sec:rel} describes the related work to our method. \cref{sec:method} presents the proposed method (RemoteMamba). \cref{sec:exp} provides extensive experiments and evaluations on benchmarks, followed by the conclusion in \cref{sec:conclusion}.

==> sections/method.tex <==
\section{METHODOLOGY} \label{sec:method}


\begin{figure*}[!htb]
    \centering
    \includegraphics[width=\linewidth]{frameworl-mambarseg.pdf}
    \caption{Framework of the proposed RemoteMamba for remote sensing image semantic segmentation. (a) RemoteMamba. (b) CSMamba Block. (c) 2D-SSM Module. }
    \label{fig:framework}
\end{figure*}

In this section, we present RemoteMamba, a mamba-based framework for remote sensing semantic segmentation, as illustrated in \cref{fig:framework}. We begin with the preliminaries of the state space model (\cref{sec3.1}), followed by a detailed description of the basic architecture, with  (\cref{sec3.2}). Finally, we conclude with the training objectives (\cref{sec3.3}).

\subsection{Preliminaries} \label{sec3.1}
In this section, we first provide a comprehensive explanation of the state space models (SSMs). SSMs aim to build a linear time-invariant (LTI) system, which maps the 1D sequence $x(t) \in \mathbb{R}^{L}$ to response $y(t) \in \mathbb{R}^{L}$, for $t$ is the time step. SSMs are typically formulated as linear ordinary differential equations (ODEs): 

\begin{equation}
\begin{aligned}
\label{eq:ssm}
    h'(t)&={\rm \textbf{A}}h(t)+{\rm \textbf{B}}x(t),\\
    y(t)&={\rm \textbf{C}}h(t)+{\rm \textbf{D}}x(t),
\end{aligned}
\end{equation}
where ${\rm \textbf{A}} \in \mathbb{R}^{L\times L}$, ${\rm \textbf{B}} \in \mathbb{R}^{L \times 1}$, ${\rm \textbf{C}} \in \mathbb{R}^{1\times L}$ are the parameters of a state size $L$, and the skip connection ${\rm \textbf{D}} \in \mathbb{R}$.
Then, a discretization process is applied to \cref{eq:ssm} for translating the SSMs to the deep neural network, using the zeroth-order hold rule as: 
\begin{equation}
\begin{aligned}
\label{eq:discret-ssm}
\centering
    h_k&=\overline{\rm \textbf{A}}h_{k-1}+\overline{\rm \textbf{B}}x_k,\\
    y_k&={\rm \textbf{C}}h_k+{\rm \textbf{D}}x_k. \\
    \overline{\rm \textbf{A}} &= {\rm e}^{\rm {\Delta \textbf{A}}},\\
    \overline{\rm \textbf{B}} &=({\rm {\Delta \textbf{A}}})^{-1}({\rm e^\textbf{A}}-\textbf{I})\cdot {\rm \Delta \textbf{B}}.
\end{aligned}
\end{equation}

where $\rm \Delta \in \mathbb{R}^{D}$ is the timescale parameter to transform the continuous parameters ${{\rm \textbf{A}}}$, ${{\rm \textbf{B}}}$ to discrete parameters $\overline{{\rm \textbf{A}}}$, $\overline{{\rm \textbf{B}}}$. 
However, the \cref{eq:discret-ssm} focuses on the LTI system where the parameters remain static for different inputs. 

To expand SSMs for long-sequence modeling more flexible, recent Mamba \cite{gu2023mamba} develops a selective scan mechanism (S6) and the hardware acceleration algorithm for projecting the $\overline{\rm \textbf{B}}$, ${\rm \textbf{C}}$ and $\rm \Delta$ from the input data  $x \in \mathbb{R} ^ {B \times L \times D}$. In this paper, we also incorporate the S6 to capture the contextual information embedded in the input.


\subsection{Framework} \label{sec3.2}
% Our proposed RemoteMamba mainly consists of three parts: the CNN-based encoder, the MSAA module, and the CSMamba decoder blocks. The CNN-based encoder \textit{i.e.} ResNet is used to extract the multi-level features, including high-level that contains semantic information and low-level that contains textual features. The CSMamba Decoder is consisted of CSMamba blocks, used to establish the local textual and global contextual information. The MSAA module is used to aggregate the multi-level feature from the ResNet encoder, providing complementary information fusion like UNet to the CSMamba Decoder.

Our RemoteMamba framework shown in \cref{fig:framework}~(a) is articulated into three core components: a CNN-based encoder, the MSAA module, and the CSMamba-based decoder. Specifically, the encoder employs ResNet to distill multi-level features, encapsulating both high-level semantic and low-level textual characteristics. The MSAA module orchestrates the fusion of these multi-level features, replacing the UNet's vanilla skip connection and enhancing the decoder's capability. Within the CSMamba decoder, the assembly of CSMamba blocks is strategically designed to synergize local textual nuances with overarching contextual insights, establishing a comprehensive semantic understanding.


\subsubsection{CSMamba Block}
% Large-scale remote sensing semantic segmentation relies on the global-local information modeling . Although the recent transformer architecture that utilizes the self-attention mechanism \cite{vit,liu2021swin} shows great power on visual tasks, they often fall into the square time complexity. 

% 是否将其转移到introduction进行阐述？
Large-scale RS semantic segmentation benefits from models that integrate both global and local information processing capabilities \cite{wang2022unetformer, wu2023cmtfnet}. Recent advancements, including transformer architectures \cite{vit,liu2021swin} utilizing self-attention mechanisms, have demonstrated significant efficacy in various visual tasks. However, these models often encounter a limitation in the form of square time complexity, which poses challenges for scalability and efficiency in processing large-scale RS images. This underscores the need for innovative approaches that maintain the strengths of transformers while mitigating their computational demands.

Motivated by the success of Mamba in long-range modeling with linear complexity, we introduce the Vision State-Space Module to the remote sensing semantic segmentation area. Following~\cite{liu2024vmamba}, the input feature $X \in \mathbb{R}^{H \times W \times C}$ will go through two parallel branches. In the first branch, the feature channel is expanded to $\lambda C$ by a linear layer, where $\lambda$ is a pre-defined channel expansion factor, followed by a depth-wise convolution, SiLU~\cite{shazeer2020glu} activation function, together with the 2D-SSM layer and Layernorm. In the second branch, the features channel is also expanded to $\lambda C$ with a linear layer followed by the SiLU activation function. After that, features from the two branches are aggregated with the Hadamard product. Finally, the channel number is projected back to $C$ to generate output $X_{out}$ with the same shape as input:
\begin{equation} \label{eq:vssm}
\centering
\begin{aligned}
    &X_1 = \mathrm{LN(2D\text{-}SSM(SiLU(DWConv(Linear}(X)))))\\
    &X_2 = \mathrm{SiLU(Linear}(X)),\\
    &X_{out} = \mathrm{Linear}(X_1 \odot X_2),
\end{aligned}
\end{equation}

where DWConv represents depth-wise convolution, and $\odot$ denotes the Hadamard product.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{msa.pdf}
    \caption{The Multi-Scale Attention Aggregation (MSAA) module.}
    \label{fig:msa}
\end{figure}

\textbf{2D Selective Scan Module.} The original Mamba model \cite{gu2023mamba} is proposed to process the 1-D data via sequential selective scanning. While this aligns well with the NLP tasks, it presents notable challenges when applied to non-causal data forms, such as images. In this paper, we follow the approach proposed by \cite{liu2024vmamba}, incorporating the 2D Selective Scan Module (2D-SSM) for image semantic segmentation. As illustrated in \cref{fig:framework}.(c), 2D-SSM first flattens the image feature to the 1D sequence and then scans the 1D sequence via different directions: from top-left to bottom-right, bottom-right to top-left, top-right to bottom-left, and bottom-left to top-right. In this way, 2D-SSM can inherently capture the long-range dependency of each direction sequence via the discrete selective state-space model. Then all direction sequences are merged by rearrange to recover the 2D structure.

\subsubsection{Multi-Scale Attention Aggregation.}
\cref{fig:msa} illustrates the multi-scale fusion and channel aggregation processes for remote sensing image feature refinement. For the output of multi-stage ResNet encoder $\mathbb{F}_{1}$, $\mathbb{F}_{2}$, and $\mathbb{F}_{3}$, we firstly concat them to the corresponding stage $\hat{F}_{i} = \text{Concat}(\mathbb{F}_{i}, \mathbb{F}_{i-1}, \mathbb{F}_{i+1})$, and reshape xxx. The concat feature $\hat{\mathbb{F}} \in \mathcal{R}^{C_1 \times H \times W}$ then is passed into the MSAA for further feature refinement. 

The MSAA consists of the dual path for feature aggregation, \textit{e.g.} Spatial and Channel. For spatial refinement, $\hat{\mathbb{F}}$ first undergoes a $1 \times 1 Conv$ for channel projection, with a factor $\alpha$, that the channel $C_1$ is projected into $C_2$, as $C_2 = \frac{C_1}{\alpha}$. Then we employ a multi-scale fusion to involve convolutions with different kernel sizes and then sum up the results: 
\begin{align*}
F_{ms} = \sum_{k \in \{3,5,7\}} \text{Conv}_{k \times k}(\hat{F})
\end{align*}
Then a spatial aggregation module is applied to aggregate the spatial feature using the mean pooling and max pooling layers followed by a $7\times7$ convolution and element-wise multiplication with the sigmoid activation of the pooled feature map. 
\begin{align*}
F_{spatial} = \sigma(\text{Conv}_{1 \times 1}(\text{Pool}(F))) \odot F
\end{align*}
where \( \sigma \) denotes the sigmoid activation function, \( \odot \) denotes element-wise multiplication, and \( + \) denotes element-wise addition.

In parallel to the spatial path, the MSAA also employs a channel aggregation process. Here, the original input feature map $\hat{F}$ is first subjected to global average pooling, reducing its dimensions to \( C_1 \times 1 \times 1 \), which is a compressed form capturing channel-wise statistics. This vector then passes through a \( 1 \times 1 \) convolution and a ReLU activation function, and subsequently, another \( 1 \times 1 \) convolution, to generate a channel attention map of the same dimensions (\( C_1 \times 1 \times 1 \)).
\begin{align*}
F_{channel} = \text{Conv}_{1 \times 1}(\text{ReLU}(\text{Conv}_{1 \times 1}(\text{AvgPool}(F))))
\end{align*}


Lastly, the channel attention map is then expanded back to the spatial dimensions of the input feature map and is element-wise multiplied by the feature map that has been spatially attended to. 
\begin{align*}
F_{out} = F_{spatial} + F_{channel}
\end{align*}

With the assistance of MSAA, the feature contains rich spatially and channel-wise refined features, poised for subsequent layers of the neural network.


\subsubsection{Multi-Output Supervision.}

Previous works have verified the intermediate supervision is xx for segmentation \cite{xxx}. Unlike \cite{wang2022unetformer} fuses the multi-level features for intermediate predictions, our MamabaRSeg applies the intermediate supervision for each CSMamba block. 

The intermediate output of $i_{th}$ CSMamba block is:
\begin{equation} \label{eq:multi-output}
    p_{i} = \text{Conv} (F_{cs})
\end{equation}

where $F_{cs}$ is the feature of $i_{th}$ CSMamba block. The $\text{Conv}$ module is used for mapping the features to the output $C$ channels class prediction map. 

\subsection{Training Objectives}  \label{sec3.3}
In the training stage, we employ both the primary feature mask output refine head and the auxiliary multi-output refinement head to optimize the CSMamba blocks, as shown in \cref{fig:framework}. The principal loss is a combination of a dice loss and a cross-entropy loss, which can be formulated as:

\begin{equation}
\begin{aligned}
\mathcal{L}_{ce} & =-\frac{1}{N} \sum_{n=1}^N \sum_{k=1}^K p_k^n \log \hat{p_k^{n}} \\ 
\mathcal{L}_{dice} & =1-\frac{2}{N} \sum_{n=1}^N \sum_{k=1}^K \frac{\hat{p_k^n} p_k^n}{\hat{p_k^n} + p_k^n} \\
\mathcal{L}_{p} &= \mathcal{L}_{ce} + \mathcal{L}_{dice}
\end{aligned}
\end{equation}
where $N$ and $K$ denote the number of training samples and the number of categories. $\hat{p^n}$ and ${p^n}$ denote the predicted output and the one-hot encoding of the ground truth, respectively. $\hat{p_k^n}$ denotes the confidence of category $K$ in sample $N$.

To better combine the primary and auxiliary losses, we further multiply the auxiliary losses
by the factor $\lambda$. In our experiments, we set $\lambda$ to 0.4. So that
our overall training objectives are defined as follows:

\begin{equation}
    \mathcal{L} = \mathcal{L}_{p} + \lambda \mathcal{L}_{aux}
\end{equation}


==> sections/relatedwork.tex <==
\section{Related Works}\label{sec:rel}
\subsection{Remote Sensing Image semantic Segmentation}

% ESDINet proposes an efficient shallow-deep interaction network for semantic segmentation of high-resolution aerial images, focusing on extracting low-level spatial and high-level semantic information quickly through a novel lightweight dual-branch architecture.

% Hybrid Attention Fusion introduces a Transformer-based decoder that embeds a hybrid attention mechanism into the Transformer, utilizing ResNet50 as an encoder to enhance semantic segmentation by aggregating features and improving global context understanding​​.

% Large Selective Kernel Network (LSKNet) addresses remote sensing object detection by dynamically adjusting its spatial receptive field to better model the context of various objects, a novel approach in utilizing large and selective kernel mechanisms​​.

% Self-Correlation and Cross-Correlation Learning tackles few-shot remote sensing image semantic segmentation by leveraging self-correlation and cross-correlation between support and query images, enhancing generalization and addressing the variance in appearance and scales of geographic objects​​.

% Swin Transformer Embedding UNet combines the Swin Transformer's global modeling capabilities with the classical CNN-based UNet for remote sensing image semantic segmentation, introducing a spatial interaction module and a feature compression module to improve feature representation and segmentation accuracy​​.

% Bilateral Awareness Network for very fine resolution urban scene images, combines a Transformer backbone for long-range relationships and convolution operations for fine-grained details, integrating both via an attentional feature aggregation module​​.

% UNetFormer develops an UNet-like Transformer for efficient semantic segmentation of remote sensing urban scene imagery, choosing ResNet18 as the encoder and innovating with a global-local attention mechanism to efficiently model both global and local information​​.

% Semantic Labeling Using EfficientUNets and Transformers proposes a novel model that integrates CNNs with transformers for semantic segmentation, leveraging both local and global feature extraction techniques to handle the large size and high spatial resolution of remote sensing images​​.

% These works collectively emphasize the integration of Transformer-based models with convolutional neural networks (CNNs) and innovative attention mechanisms to address the challenges of semantic segmentation in remote sensing imagery. The commonality lies in the pursuit of capturing both local details and global context effectively, while differences are noted in the specific architectural innovations and application focuses, ranging from few-shot learning and object detection to comprehensive semantic segmentation tasks.

% The documents collectively present advancements in semantic segmentation for remote sensing images, leveraging Transformer models, CNNs, and innovative network architectures:
% A novel Transformer-based scheme utilizes Swin Transformer and DCFAM for fine-resolution imagery, enhancing segmentation accuracy through multi-scale semantic feature capture.
% ABCNet introduces an Attentive Bilateral Contextual Network to efficiently segment fine-resolution remote sensing images, focusing on context awareness and attention mechanisms.
% CMTFNet merges CNNs with Multiscale Transformers to balance local feature extraction and global context understanding, improving semantic segmentation performance.
% CM-Unet innovates on the U-Net architecture for remote sensing image segmentation, incorporating improved feature extraction and processing techniques.
% CTMFNet combines CNNs and Transformers for a multiscale fusion network, targeting the unique challenges of urban scene imagery segmentation.
% DHRNet proposes a Dual-Branch Hybrid Reinforcement Network, optimizing the integration of spatial and semantic information for enhanced segmentation results.
% These works underline the shift towards hybrid models that integrate the strengths of CNNs and Transformers, aiming to capture detailed local features and global context for accurate remote sensing image segmentation.

The semantic segmentation of remote sensing imagery generally revolves three primary approaches: CNN-based, Transformer-based and CNN-Transformer hybrid. The CNN-based methods mainly leverage the FCNs \cite{huang2017densely, kemker2018algorithms} or encoder-decoder architecture \cite{diakogiannis2020resunet} to extract multi-scale features and gradually collect the semantic information. OCNN \cite{zhang2018object} introduces the object-based CNN framework for land use classification across complex scenarios, marking a significant advancement in the field. SDNF \cite{mi2020superpixel} and ESCNet \cite{zhang2021escnet} further innovate by developing semantic segmentation networks that leverage superpixels to enhance the segmentation process.LSKNet \cite{li2023large} addresses remote sensing object detection by dynamically adjusting its spatial receptive field to better model the context of various objects, utilizing large and selective kernel mechanisms. However, due to the complex buildings, trees, and various objects \textit{e.g.} cars, humans, the inherent small receptive field of CNN kernels is limited to capture the global long-range dependencies. 

With the rise of transformer \cite{vaswani2017attention} and vision transformer \cite{dosovitskiy2020image} that have a powerful performance on sequence-to-sequence modeling, the transformer-based methods focus on designing various attention mechanisms. Segmenter and SegFormer \cite{strudel2021segmenter, xie2021segformer} employ the entire transformer-blocks encoder-decoder network for building the long-range dependencies. MMT \cite{xu2023mmt} employs the mixed-mask transformer to assist the intra-class and inter-class correlations learning. Although the transformer-based methods can capture the long-range dependencies, they are sometimes at cost time complexity.

The last CNN-transformer hybrid mixture methods mainly adapt the CNNs as the encoder to pre-extract the multi-level image features and employ the various transformer blocks to build a segmentation decoder. SwinUNet \cite{he2022swin} utilizes Swin Transformer and CNN for fine-resolution imagery, enhancing segmentation accuracy through multi-scale semantic feature capture. DHRNet proposes a dual-branch hybrid reinforcement network, optimizing the integration of spatial and semantic information for enhanced segmentation results. BANet \cite{banet} constructs two feature extraction paths: one path uses CNN to extract local texture features and the other path uses the transformer to capture long-range dependencies. UNetFormer \cite{wang2022unetformer} develops an UNet-like Transformer for efficient semantic segmentation of remote sensing urban scene imagery, choosing ResNet18 as the encoder and innovating with a global-local attention mechanism to efficiently model both global and local information. CTMFNet \cite{song2022ctmfnet} combines CNNs and Transformers for a multiscale fusion network, targeting the unique challenges of urban scene imagery segmentation. ESDINet \cite{ESDINet} proposes an efficient shallow-deep interaction network for semantic segmentation of high-resolution aerial images, focusing on extracting low-level spatial and high-level semantic information quickly through a novel lightweight dual-branch architecture.

Our proposed RemoteMamba also utilizes CNN's textual feature extraction capabilities and the Mamba's long-range dependencies modeling with linear time. We first introduce the CNN-Mamba hybrid architecture for efficient RS image semantic segmentation. 



\subsection{State Space Models}
Drawing from the control theory~\cite{kalman1960new}, State Space Models (SSMs) have recently been introduced to deep learning as an alternative for CNNs and transformers in modeling long-range dependencies. The Structured State-Space Sequence model (S4) \cite{mehta2022long} employs a linear state space for contextualization and shows strong performance on various sequence modeling tasks, especially with lengthy sequences. To accelerate the computation, \cite{gu2022parameterization, gu2022train,gupta2022diagonal} develops the efficient matrix calculation. \cite{mehta2022long} builds the Gated State Space layer on S4 by introducing more gating units to improve the expressivity. Subsequently, \cite{smith2022simplified} proposes the S5 layer that involves MIMO SSM and efficient parallel scan into the S4 layer. Then \cite{islam2022long, nguyen2022s4nd, islam2023efficient} employs the S4 layer and its variants into computer vision, achieving preliminary success. 

Recently, \cite{gu2023mamba} proposes a data-dependent Selective State Model layer with linear time computation and efficient training process via integrating selection mechanism and hardware-aware algorithms, which have achieved great performance in NLP tasks. Building on the success of Mamba, \cite{pioro2024moe, wang2024graph} employs the Mixture of Experts and Graph Node with Mamba to explore the potential of replacing the transformer in various tasks. Furthermore, \cite{liu2024vmamba, zhu2024vision} utilize the bidirectional vision select module and cross-scan module respectively to extend Mamba from 1D sequence processing to 2D vision level. In this work, we also inherit from the powerful performance of Mamba, transferring it to the more challenging scenario, \textit{i.e.} RS image semantic segmentation. To further extract the rich global and complicated textual information in RS images, we design a channel and spatial Mamba (CSMamba) block as a base block of the decoder to capture the long-range dependencies.
